Rainfall-runoff prediction using a Gustafson-Kessel clustering based Takagi-Sugeno Fuzzy model

A rainfall-runoff model predicts surface runoff either using a physically-based approach or using a systems-based approach. Takagi-Sugeno (TS) Fuzzy models are systems-based approaches and a popular modeling choice for hydrologists in recent decades due to several advantages and improved accuracy in prediction over other existing models. In this paper, we propose a new rainfall-runoff model developed using Gustafson-Kessel (GK) clustering-based TS Fuzzy model. We present comparative performance measures of GK algorithms with two other clustering algorithms: (i) Fuzzy C-Means (FCM), and (ii)Subtractive Clustering (SC). Our proposed TS Fuzzy model predicts surface runoff using: (i) observed rainfall in a drainage basin and (ii) previously observed precipitation flow in the basin outlet. The proposed model is validated using the rainfall-runoff data collected from the sensors installed on the campus of the Indian Institute of Technology, Kharagpur. The optimal number of rules of the proposed model is obtained by different validation indices. A comparative study of four performance criteria: RootMean Square Error (RMSE), Coefficient of Efficiency (CE), Volumetric Error (VE), and Correlation Coefficient of Determination(R) have been quantitatively demonstrated for each clustering algorithm.

==> name.tex <==
\subsection{Validation for a short duration large storm event (Data Set 3)}\label{DATA SET 3}
%%%%%%%%%%%%%%%%%% D S 5 Dimensional%%%%%%%
In this subsection, G-K, FCM and SC algorithms based TS fuzzy models are constructed for eleven mathematical models $(M_1, M_2,..., M_{11})$ for both training (Data Set 1) and validation of a short duration large storm event (Data Set 3).

Table \ref{GK fuzzy model_DS3} specifies the performances of all the models ($M_1$ to $M_{11}$) for dimensional and dimensionless input (Data Set 3) using GK algorithm. The $M_4$ model gives better performance than the other ten models, shown in Table \ref{GK fuzzy model_DS3} for both the dimensional and dimensionless input.


\begin{table}[h!]\centering
\centering \caption{Model Performance by GK based Fuzzy Model for dimensional and dimensionless input of Data Set 3} \label{GK fuzzy model_DS3}
\resizebox{9cm}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline \multicolumn{5}{|l|}{Training} &
\multicolumn{4}{l|}{Validation} \\ \hline
 Models  & RMSE & VE & CE & R & RMSE       & VE & CE & R\\ \hline
$M_1$   &39.97  &16.2   &0.73   &0.86   &664.26 &133.46 &-20.14 &0.44   \\  \hline
$M_1(N)$    &0.12   &17.83  &0.71   &0.85   &0.34   &39.99  &-0.96  &0.7    \\  \hline
$M_2$   &42.14  &18.42  &0.7    &0.84   &170.69 &37.68  &-0.4   &0.39   \\  \hline
$M_2(N)$    &0.12   &17.25  &0.73   &0.85   &0.31   &39.21  &-0.6   &0.62   \\  \hline
$M_3$   &43.94  &19.13  &0.68   &0.82   &147.78 &30.17  &-0.05  &0.44   \\  \hline
$M_3(N)$    &0.12   &18.33  &0.7    &0.83   &0.46   &52.81  &-2.45  &0.4    \\  \hline
$M_4$   &0.02   &0.01   &1  &1  &0.39   &0.02   &1  &1  \\  \hline
$M_4(N)$    &0.01   &0.99   &1  &1  &0.01   &2.5    &0.99   &0.99   \\  \hline
$M_5$   &11.84  &4.49   &0.98   &0.99   &72.42  &15.76  &0.75   &0.94   \\  \hline
$M_5(N)$    &0.03   &3.63   &0.98   &0.99   &0.16   &21.25  &0.55   &0.81   \\  \hline
$M_6$   &11.4   &4.49   &0.98   &0.99   &66.34  &12.34  &0.79   &0.92   \\  \hline
$M_6(N)$    &0.03   &3.97   &0.98   &0.99   &0.1    &11.18  &0.83   &0.92   \\  \hline
$M_7$   &10.94  &3.88   &0.98   &0.99   &74.95  &16.43  &0.73   &0.93   \\  \hline
$M_7(N)$    &0.03   &3.89   &0.98   &0.99   &0.27   &33.42  &-0.18  &0.67   \\  \hline
$M_8$   &10.56  &3.9    &0.98   &0.99   &71.1   &13.27  &0.76   &0.92   \\  \hline
$M_8(N)$    &0.03   &3.62   &0.98   &0.99   &0.17   &21.38  &0.5    &0.82   \\  \hline
$M_9$   &11.29  &4.44   &0.98   &0.99   &71.09  &13.41  &0.76   &0.88   \\  \hline
$M_9(N)$    &0.02   &3.28   &0.99   &0.99   &0.11   &13.2   &0.81   &0.92   \\  \hline
$M_{10}$    &9.94   &3.55   &0.98   &0.99   &381.27 &78.3   &-5.96  &0.03   \\  \hline
$M_{10}(N)$ &0.03   &3.44   &0.98   &0.99   &0.15   &18.52  &0.62   &0.86   \\  \hline
$M_{11}$    &10.74  &4.16   &0.98   &0.99   &69.2   &13.15  &0.77   &0.89   \\  \hline
$M_{11}(N)$ &0.03   &3.31   &0.98   &0.99   &0.38   &32.7   &-1.42  &0.61   \\  \hline
\end{tabular}}
\end{table}

The $M_4$ model performances for the training dataset (Data Set 1) and validation dataset (Data Set 3) using GK algorithm are shown in the Figure \ref{GK4_trainDS3} and Figure \ref{GK4_testDS3}.


\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/GKtrainingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model trained by G-K based Fuzzy Model}
\label{GK4_trainDS3}
\end{figure}
\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/GKtestingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model validated for Data Set 3 by G-K based Fuzzy Model }
\label{GK4_testDS3}
\end{figure}


Table \ref{SC fuzzy model_DS3} specifies the performances of all the models ($M_1$ to $M_{11}$) for dimensional and dimensionless input (Data Set 3) using SC algorithms. The $M_4$ model gives better performance than the other ten models, shown in Table \ref{SC fuzzy model_DS3} for both the dimensional and dimensionless input.


\begin{table}[h!]\centering
\centering \caption{Model Performance by SC based Fuzzy Mode for dimensional and dimensionless input of Data Set 3} \label{SC fuzzy model_DS3}
\resizebox{9cm}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline \multicolumn{5}{|l|}{Training} &
\multicolumn{4}{l|}{Validation} \\ \hline
 Models  & RMSE & VE & CE & R & RMSE       & VE & CE & R\\ \hline
$M_1$   &41.66  &17.62  &0.71   &0.84   &245.09 &59.65  &-1.88  &0.76   \\  \hline
$M_1(N)$    &0.14   &22.46  &0.63   &0.79   &0.26   &33.04  &-0.12  &0.41   \\  \hline
$M_2$   &39.39  &16 &0.74   &0.86   &8984.49    &1416.15    &-3866.02   &-0.42  \\  \hline
$M_2(N)$    &0.12   &18.86  &0.7    &0.84   &0.4    &47.11  &-1.63  &0.29   \\  \hline
$M_3$   &42.01  &16.9   &0.71   &0.84   &11825.57   &1814.7 &-6698.37   &-0.21  \\  \hline
$M_3(N)$    &0.13   &18.84  &0.67   &0.82   &0.23   &28.33  &0.15   &0.61   \\  \hline
$M_4$   &0.75   &0.29   &1  &1  &195.94 &17.81  &-0.69  &0.22   \\  \hline
$M_4(N)$    &0.01   &1.38   &1  &1  &0.02   &2.02   &0.99   &1  \\  \hline
$M_5$   &11.05  &4.06   &0.98   &0.99   &87.61  &17.66  &0.63   &0.92   \\  \hline
$M_5(N)$    &0.03   &4.52   &0.98   &0.99   &0.13   &14.58  &0.71   &0.92   \\  \hline
$M_6$   &10.81  &4.35   &0.98   &0.99   &113.09 &21.61  &0.39   &0.83   \\  \hline
$M_6(N)$    &0.03   &4.32   &0.98   &0.99   &0.14   &16.29  &0.67   &0.92   \\  \hline
$M_7$   &11.05  &4.21   &0.98   &0.99   &150.25 &32.38  &-0.08  &0.74   \\  \hline
$M_7(N)$    &0.03   &4.11   &0.98   &0.99   &0.13   &13.88  &0.71   &0.91   \\  \hline
$M_8$   &10.35  &4.07   &0.98   &0.99   &70.49  &15.85  &0.76   &0.92   \\  \hline
$M_8(N)$    &0.03   &4.15   &0.98   &0.99   &0.14   &15.51  &0.69   &0.91   \\  \hline
$M_9$   &10.98  &4.27   &0.98   &0.99   &117.33 &21.42  &0.34   &0.76   \\  \hline
$M_9(N)$    &0.03   &4.34   &0.98   &0.99   &0.14   &17.4   &0.66   &0.87   \\  \hline
$M_{10}$    &10.99  &4.2    &0.98   &0.99   &109.47 &22.42  &0.43   &0.83   \\  \hline
$M_{10}(N)$ &0.03   &4.24   &0.98   &0.99   &0.1    &13.11  &0.83   &0.94   \\  \hline
$M_{11}$    &9.08   &3.31   &0.99   &0.99   &165.24 &34.82  &-0.31  &0.64   \\  \hline
$M_{11}(N)$ &0.03   &3.33   &0.99   &0.99   &0.16   &19.43  &0.56   &0.86   \\  \hline
\end{tabular}}
\end{table}

The $M_4$ model performances for the training dataset (Data Set 1) and validation dataset (Data Set 3) using SC algorithm are shown in the Figure \ref{SC4_trainDS3} and Figure \ref{SC4_testDS3}.

\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/SCtrainingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model trained by SC based Fuzzy Model}
\label{SC4_trainDS3}
\end{figure}
\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/SCtestingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model validated for Data Set 3 by SC based Fuzzy Model }
\label{SC4_testDS3}
\end{figure}



Table \ref{FCM fuzzy model_DS3} specifies the performances of all the models ($M_1$ to $M_{11}$) for dimensional and dimensionless input (Data Set 3) using FCM algorithm . The $M_4$ model gives better performance than the other ten models, shown in Table \ref{FCM fuzzy model_DS3} for both the dimensional and dimensionless input.


\begin{table}[h!]\centering
\centering \caption{Model Performance by FCM based Fuzzy Model for dimensional and dimensionless input of Data Set 3} \label{FCM fuzzy model_DS3}
\resizebox{9cm}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline \multicolumn{5}{|l|}{Training} &
\multicolumn{4}{l|}{Validation} \\ \hline
 Models  & RMSE & VE & CE & R & RMSE       & VE & CE & R\\ \hline
$M_1$   &45.07  &20.56  &0.66   &0.81   &292.18 &63.19  &-3.09  &0.46   \\  \hline
$M_1(N)$    &0.07   &0.07   &10.85  &0.91   &0.95   &0.26   &31.62  &-0.09  \\  \hline
$M_2$   &44.01  &19.59  &0.68   &0.82   &842.53 &158.44 &-33.01 &0.46   \\  \hline
$M_2(N)$    &0.06   &0.06   &9.73   &0.92   &0.96   &0.26   &34.82  &-0.15  \\  \hline
$M_3$   &46.16  &20.44  &0.65   &0.8    &821.98 &151.61 &-31.37 &0.45   \\  \hline
$M_3(N)$    &0.06   &0.06   &9.67   &0.92   &0.96   &0.27   &35.55  &-0.21  \\  \hline
$M_4$   &4.69   &1.42   &1  &1  &11.27  &2.16   &0.99   &1  \\  \hline
$M_4(N)$    &0.02   &0.02   &1.28   &1  &1  &0.02   &2.23   &1  \\  \hline
$M_5$   &11.98  &4.54   &0.98   &0.99   &131.59 &27.4   &0.17   &0.74   \\  \hline
$M_5(N)$    &0.03   &0.04   &4.84   &0.98   &0.99   &0.12   &15.82  &0.75   \\  \hline
$M_6$   &10.47  &4.33   &0.98   &0.99   &141.28 &28.3   &0.04   &0.75   \\  \hline
$M_6(N)$    &0.03   &0.03   &4.5    &0.98   &0.99   &0.12   &13.79  &0.77   \\  \hline
$M_7$   &11.03  &4.28   &0.98   &0.99   &218.74 &45.96  &-1.29  &0.38   \\  \hline
$M_7(N)$    &0.03   &0.03   &4.58   &0.98   &0.99   &0.25   &30.78  &-0.01  \\  \hline
$M_8$   &10.28  &4.17   &0.98   &0.99   &193.75 &35.52  &-0.8   &0.56   \\  \hline
$M_8(N)$    &0.03   &0.03   &4.02   &0.98   &0.99   &0.14   &17.24  &0.65   \\  \hline
$M_9$   &11.47  &4.53   &0.98   &0.99   &130.47 &26.61  &0.18   &0.83   \\  \hline
$M_9(N)$    &0.03   &0.03   &4.29   &0.98   &0.99   &0.12   &15.22  &0.74   \\  \hline
$M_{10}$    &10.58  &4.33   &0.98   &0.99   &134.85 &28.97  &0.13   &0.76   \\  \hline
$M_{10}(N)$ &0.03   &0.03   &4.15   &0.98   &0.99   &0.12   &15.33  &0.74   \\  \hline
$M_{11}$    &10.2   &4.06   &0.98   &0.99   &125.7  &26.71  &0.24   &0.78   \\  \hline
$M_{11}(N)$ &0.03   &0.03   &4.13   &0.98   &0.72   &0.13   &15.68  &0.72   \\  \hline
\end{tabular}}
\end{table}

The $M_4$ model performances for the training dataset (Data Set 1) and validation dataset (Data Set 3) using FCM algorithm are shown in the Figure \ref{FCM4_trainDS3} and Figure \ref{FCM4_testDS3}.


\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/FCMtrainingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model trained by FCM based Fuzzy Model}
\label{FCM4_trainDS3}
\end{figure}
\begin{figure}[h!] \centering
%\hspace*{-10mm}
\includegraphics[width=70mm]{figs/Figures/FCMtestingDS3.eps}
\caption{Observed vs Estimated pressure head (before 60 sec) for $M_4$ Model validated for Data Set 3 by FCM based Fuzzy Model }
\label{FCM4_testDS3}
\end{figure}

From the above discussions and observations from the model performances, it can be concluded that the G-K based TS fuzzy model gives better performance (considering all the eleven models) than that of the FCM and SC based fuzzy models. We observed that three clustering algorithms based TS fuzzy model cannot perform satisfactorily for the first three models ($M_1$ to $M_3$). Hence, the model performances are significantly improved using the observed runoff at the previous time interval as inputs along with the rainfall events (in the present and past time interval). The $M_4$ model gives the best model performance out of all the eleven models, obtained by all the fuzzy clustering algorithms. The reason behind a significantly better performances of $M_4$ model in both dimensional and dimensionless dataset can be explained from a physical perspective. For each model, described in this article, lag-time or basin lag (i.e. the time from the center of mass of excess rainfall to the hydrograph peak) has been removed from each of input rainfall data-set. Hence, the channel flow at any given time interval depends on the accumulated surface water that is flowing into the channel due to present rainfall (due to conservation of mass and momentum) and channel flow in the previous time instant (due to the continuity equation). Considering the structure of the $M_4$ model, it is interesting to note that the chosen input variables (viz. present input and runoff in the previous time instant) are direct consequences of the conservation of mass and momentum law and continuity equation. Hence the $M_4$ model is showing the better statistical values than the other ten models.


